Semantic uncertainty intervals for disentangled latent spaces

Meaningful uncertainty quantification in computer vision requires reasoning about semantic information -- say, the hair color of the person in a photo or the location of a car on the street. To this end, recent breakthroughs in generative modeling allow us to represent semantic information in disentangled latent spaces, but providing uncertainties on the semantic latent variables has remained challenging. In this work, we provide principled uncertainty intervals that are guaranteed to contain the true semantic factors for any underlying generative model. The method does the following: (1) it uses quantile regression to output a heuristic uncertainty interval for each element in the latent space (2) calibrates these uncertainties such that they contain the true value of the latent for a new, unseen input. The endpoints of these calibrated intervals can then be propagated through the generator to produce interpretable uncertainty visualizations for each semantic factor. This technique reliably communicates semantically meaningful, principled, and instance-adaptive uncertainty in inverse problems like image super-resolution and image completion.

==> algorithms/all_algorithms.tex <==
\begin{minipage}{0.46\textwidth}
    \begin{algorithm}[H]
        \caption{Quantile GAN encoder training}
        \label{alg:gqan-encoder-training}
        \begin{algorithmic}
           \STATE {\bfseries Input:} training dataset $\mathcal{D}$, risk level $\alpha$, number of epochs $E$, fixed generator $G$
           \STATE {\bfseries Output:} trained functions $f,q_{\frac{\alpha}{2}},$ and $q_{1-\frac{\alpha}{2}}$.
           \STATE $f,q_{\frac{\alpha}{2}},$ and $q_{1-\frac{\alpha}{2}} \gets$ random model initialization
           \FOR{$e=1$ {\bfseries to} $E$}
              \STATE \texttt{loss} $\gets 0$
              \FOR{$(X^{\rm train},Z^{\rm train})$ {\bfseries in} $\mathcal{D}$}
                  \STATE \texttt{L1} $\gets \mathcal{L}_{\rm pred}\big(f(X^{\rm train}\big),Z^{\rm train})$ 
                  
                  \STATE \texttt{L2} $\gets \mathcal{L}^{\frac{\alpha}{2}}_{\rm q}\big(q_{\frac{\alpha}{2}}(X^{\rm train}\big),Z^{\rm train})$
                  
                  \STATE \texttt{L3} $\gets \mathcal{L}^{1-\frac{\alpha}{2}}_{\rm q}\big(q_{1-\frac{\alpha}{2}}(X^{\rm train}\big),Z^{\rm train})$
                  
                  \STATE \texttt{loss += L1 + L2 + L3}
              \ENDFOR
              \STATE \texttt{loss.backward()}
           \ENDFOR
        
        \end{algorithmic}
    \end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.46\textwidth}
\begin{algorithm}[H]
    \caption{RCPS calibration}
   \label{alg:rcps-calibration}
    \begin{algorithmic}
       \STATE {\bfseries Input:} calibration data $\big\{(X_i,Z_i)\big\}_{i=1}^n$, risk level $\alpha$, error level $\delta$, step size $d\lambda$, maximum value $\lambda_{\rm max}$
       \STATE {\bfseries Output:} calibrated parameter $\lhat$

       \STATE $\lambda \gets \lambda_{\rm max}$
       \REPEAT
           \STATE $r \gets \hat{R}^+(\lambda)$ \COMMENT{see~\eqref{eq:hoeffding}}
           \STATE $\lambda \gets \lambda - d\lambda$
       \UNTIL{$r > \alpha$}
       \STATE $\lhat \gets \lambda + d\lambda$ \COMMENT{overshot by one step.}
    \end{algorithmic}
\end{algorithm}
\end{minipage}

==> algorithms/rcps-calibration.tex <==
\begin{algorithm}[tb]
   \caption{RCPS calibration}
   \label{alg:rcps-calibration}
    \begin{algorithmic}
       \STATE {\bfseries Input:} calibration data $\big\{(X_i,Z_i)\big\}_{i=1}^n$, risk level $\alpha$, error level $\delta$, step size $d\lambda$, maximum value $\lambda_{\rm max}$
       \STATE {\bfseries Output:} calibrated parameter $\lhat$

       \STATE $\lambda \gets \lambda_{\rm max}$
       \REPEAT
           \STATE $r \gets \hat{R}^+(\lambda)$ \COMMENT{see~\eqref{eq:hoeffding}}
           \STATE $\lambda \gets \lambda - d\lambda$
       \UNTIL{$r > \alpha$}
       \STATE $\lhat \gets \lambda + d\lambda$ \COMMENT{overshot by one step.}
    \end{algorithmic}
\end{algorithm}


==> changelog.tex <==
Changelog:

* Textual edits on why uncertainty on semantics is useful, introducing distribution-free risk control, and so on.
* Added a new section and results incorporating experiments on real data, with an improved model.  Included results showing how calibration changes the visualized output semantically.
* Moved experiments showcasing effect of calibration and coverage as a function of problem difficulty to the appendix.
* Added additional results to the appendix including an ablation on the feature loss and quantifying coverage and adaptivity in real data.
* Added author acknowledgement

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
